Convolutional Bipartite Attractor Networks

In human perception and cognition, a fundamental operation that brains perform is interpretation: constructing coherent neural states from noisy, incomplete, and intrinsically ambiguous evidence. The problem of interpretation is well matched to an early and often overlooked architecture, the attractor network---a recurrent neural net that performs constraint satisfaction, imputation of missing features, and clean up of noisy data via energy minimization dynamics. We revisit attractor nets in light of modern deep learning methods and propose a convolutional bipartite architecture with a novel training loss, activation function, and connectivity constraints. We tackle larger problems than have been previously explored with attractor nets and demonstrate their potential for image completion and super-resolution. We argue that this architecture is better motivated than ever-deeper feedforward models and is a viable alternative to more costly sampling-based generative methods on a range of supervised and unsupervised tasks.

==> CBAN [ARXIV - (ICLR) 2020]/helpers/custom_commands.tex <==
\newcommand{\bw}{{\ensuremath{\bm{w}}}}
\newcommand{\bh}{{\ensuremath{\bm{h}}}}
\newcommand{\bv}{{\ensuremath{\bm{v}}}}
\newcommand{\bW}{{\ensuremath{\bm{W}}}}
\newcommand{\bb}{{\ensuremath{\bm{b}}}}
\newcommand{\bx}{{\ensuremath{\bm{x}}}}
\newcommand{\by}{{\ensuremath{\bm{y}}}}
\newcommand{\T}{{\ensuremath{\mathsf{T}}}}
\newcommand*\xbar[3]{%
   \hbox{%
     \vbox{%
       \hrule height 0.5pt % The actual bar
       \kern0.2ex%         % Distance between bar and symbol
       \hbox{%
         \kern-0.15em%      % Shortening on the left side
         \ensuremath{#1}%
         \kern-0.15em%      % Shortening on the right side
       }%
     }%
   }%
  \ensuremath{{\,}^{#2}_{#3}}
} 
\newcommand{\fix}{\marginpar{FIX}}
\newcommand{\new}{\marginpar{NEW}}

\setlength{\belowdisplayskip}{1.5pt} \setlength{\belowdisplayshortskip}{1.5pt}
\setlength{\abovedisplayskip}{1.5pt} \setlength{\abovedisplayshortskip}{1.5pt}
\captionsetup{belowskip=0pt}

==> CBAN [ARXIV - (ICLR) 2020]/helpers/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> CBAN [ARXIV - (ICLR) 2020]/helpers/packages.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[hyphens]{url}            % simple URL typesetting
\usepackage[colorlinks=true,citecolor=blue]{hyperref}       % hyperlinks
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{enumitem}
\usepackage{bm}
\usepackage{float}
\usepackage{caption}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{bbold}
\usepackage{relsize}
\usepackage{multicol}
\usepackage{adjustbox}
\usepackage{wrapfig}

==> CBAN [ARXIV - (ICLR) 2020]/sections/00_abstract.tex <==
\begin{abstract}
In human perception and cognition, a fundamental operation that brains perform is \emph{interpretation}: constructing coherent neural states from noisy, incomplete, and intrinsically ambiguous evidence. The problem of interpretation is well matched to an early and often overlooked architecture, the attractor network---a recurrent neural net that performs constraint satisfaction, imputation of missing features, and clean up of noisy data via energy minimization dynamics. We revisit attractor nets in light of modern deep learning methods and propose a convolutional bipartite architecture with a novel training loss, activation function, and connectivity constraints. We tackle larger problems than have been previously explored with attractor nets and demonstrate their potential for image completion and super-resolution. We argue that this architecture is better motivated than ever-deeper feedforward models and is a viable alternative to more costly sampling-based generative methods on a range of supervised and unsupervised tasks.
\end{abstract}

==> CBAN [ARXIV - (ICLR) 2020]/sections/01_introduction_v2.tex <==
\vspace{-.10in}
\section{Introduction}
\vspace{-.04in}
Under ordinary conditions, human visual perception is quick
and accurate. Studying circumstances that give rise to slow or
inaccurate perception can help reveal the underlying mechanisms
of visual information processing. Recent investigations of 
occluded \citep{tang2018recurrent} 
and empirically challenging \citep{Kar2019} scenes have led to the 
conclusion that  recurrent brain circuits can play a critical role in object recognition. 
Further, recurrence can 
improve the classification performance of deep nets \citep{tang2018recurrent,Nayebi2018}, specifically for the same
images with which humans and animals have the most difficulty
\citep{Kar2019}.

Recurrent dynamics allow the brain to perform \emph{pattern completion}, constructing a coherent neural state from noisy, incomplete, and intrinsically ambiguous evidence.
This interpretive process is
well matched to \emph{attractor networks} (\emph{ANs})
\citep{Hopfield1982,Hopfield1984,KrotovHopfield2016,Zemel2001},
a class of dynamical neural networks that converge to fixed-point attractor states (Figure~\ref{fig:1}a). Given evidence in the form of a static input, an AN settles to an asymptotic state---an interpretation or completion---that is as consistent as possible with the evidence and with implicit knowledge embodied in the network connectivity. 
We show examples from our model in Figure~\ref{fig:1}b.
\begin{figure}[b!]
    \centering
    \includegraphics[height=1.in]{figures/figure1_v2.pdf}
    %\caption{(a) Hypothetical activation flow dynamics of an attractor net over a 2D state space: the contours depict an energy landscape, and network dynamics move downhill in energy. (b) Bipartite architecture with layer update order. (c) Convolutional architecture with optional average pooling.}
    \caption{(a) Hypothetical activation flow dynamics of an attractor net over a 2D state space; the contours depict an energy landscape. 
    (b) top-to-bottom: original image, completion, and evidence. (c) Bipartite architecture with layer update order. (d) Convolutional architecture with average pooling.}
    \label{fig:1}
\end{figure}

ANs have played a pivotal role in characterizing computation in the brain \citep{amit1992,McClelland1981}, not only
perception \citep[e.g.,][]{Sterzer2007}, but also language \citep{Stowe2018} and awareness \citep{Mozer2009}.
%Because their settling time is dependent on the consistency of evidence provided to them, ANs are suitable for explaining the variable time course of perception \citep{Sterzer2007}, but they have also been used to account for higher cognitive function such as language \citep{Stowe2018} and awareness \citep{Mozer2009}. 
We revisit attractor nets in light of  modern deep learning methods and propose a convolutional bipartite architecture 
for pattern completion tasks with a novel training loss,  activation function, and connectivity constraints. 

\vspace{-.07in}
\section{Background and Related Research}
\vspace{-.02in}

Although ANs have been mostly neglected in the recent literature, 
attractor-like dynamics can be seen in many models. For example, clustering and
denoising autoencoders are used to  clean up internal states and improve the 
robustness of deep models \citep{Liao2016,tang2018recurrent,Lamb2019}.
In a range of image-processing domains, e.g., denoising, inpainting, and super-resolution, performance gains are realized by constructing deeper and deeper architectures \citep[e.g.,][]{Lai2018}. State-of-the-art results are often obtained using deep recursive architectures that replicate layers and weights \citep{KimLeeLee2016,Tai2017}, effectively implementing an unfolded-in-time recurrent net. This approach is sensible because image processing tasks are fundamentally constraint satisfaction problems: the value of any pixel depends on the values of its neighborhood, and iterative processing is required to converge on mutually consistent activation patterns. 
Because ANs are specifically designed to address constraint-satisfaction problems, our goal is to re-examine them
from a modern deep-learning perspective.
% REMOVED FOR SPACE: in the mainstream deep learning community.
% In this article, we revisit ANs in light of modern deep-learning architectures and methodologies. We first describe our architecture, state update procedure, symmetric weight constraints, and loss functions. We then explore 
% \emph{fully connected bipartite attractor networks} (\emph{FBANs}) on simple image completion tasks before seguing into more complex image 
% completion tasks that utilize \emph{convolutional bipartite attractor networks} (\emph{CBANs}). We evaluate variations in CBAN training and show the importance of symmetry constraints. Lastly, we compare against competing models, such as VAEs and LapSRN, and show promising results for image completion and super-resolution.
    
    %Figure~\ref{fig:cifar_omni} illustrates denoising applications of our AN.
    %\item Incorporating recurrent circuits into deep object recognition models not only improves their performance, but does so specifically for images that humans and animals take the longest to process \citep{Kar2019}.

Interest in ANs seems to be narrow for two reasons.
First, in both early \citep{Hopfield1982,Hopfield1984}
and recent  \citep{Li2015,Wu2018a,Wu2018b,Chaudhuri2017} work, ANs are characterized as
content-addressable memories: activation vectors are stored
and can later be retrieved with only partial information.
However, memory retrieval does not well characterize the model's capabilities:
like its probabilistic sibling the Boltzmann machine  
\citep{Hinton2007, Welling2005}, the AN is a general computational 
architecture for supervised and unsupervised learning. 
%There is not a sharp line between retrieval of specific stored memories and interpretation of noisy and missing data. 
Second, ANs have been limited by training procedures. In Hopfield's work,
ANs are trained with a simple procedure---an outer product (Hebbian) rule---which 
cannot accommodate hidden units and the representational capacity they provide. Recent explorations 
have considered stronger training procedures 
\citep[e.g.,][]{Wu2018b,Liao2018}; however, as for all recurrent nets, training is complicated by the issue 
of vanishing/exploding gradients. To facilitate training and increase the computational power of ANs, we
propose a set of extensions to the architecture and training procedures.

ANs are related to several popular architectures. \emph{Autoencoding models} such as the VAE \citep{Kingma2013} and denoising autoencoders \citep{Vincent2008} can be viewed as approximating one step of attractor dynamics, directing the input toward the training data manifold \citep{Alain2012}. These models can be applied recursively, though convergence is not guaranteed, nor is improvement in output quality over iterations. \emph{Flow-based generative models} (FBGMs) \cite[e.g.,][]{Dinh2016} are invertible density-estimation models that can map between observations and latent states. Whereas FBGMs require invertibility of mappings, ANs require only a weaker constraint that weights in one direction are the transpose of the weights in the other direction. 

\emph{Energy-based models} (EBMs) are also density-estimation models that learn a mapping from input data to energies and are trained to assign low energy values to the data manifold \citep{LeCun2006,Han2018,Xie2016,Du2019}. Whereas AN dynamics are determined by an implicit energy function, the EBM dynamics are driven by optimizing or sampling from an explicit energy function. In the AN, lowering the energy for some states raises it for others, whereas the explicit EBM energy function requires  well-chosen negative samples to ensure it discriminates likely from unlikely states. Although the EBM and FBGM seem well suited for synthesis and generation tasks, due to their probabilistic underpinnings, we show that ANs can be used for
conditional generation (maximum likelihood completion) tasks. 

==> CBAN [ARXIV - (ICLR) 2020]/sections/02_cban_v2.tex <==
%\vspace{-.07in}
\section{Convolutional Bipartite Attractor Nets}
%\vspace{-.08in}
%\subsection{Architecture}

Various types of recurrent nets have been shown to converge to activation fixed points, including 
fully interconnected networks of asynchronous binary units 
\citep{Hopfield1982} and networks of continuous-valued units operating
in continuous time \citep{Hopfield1984}.
Most relevant to modern deep learning, \citet{Koiran1994} identified convergence conditions 
for synchronous update of continuous-valued units in discrete time:
given a network with state $\bx$, parallel updates of the full state with the standard activation rule,
\begin{equation}
\bx \leftarrow f(\bx \bW + \bb),
\label{eq:xiupdate}
\end{equation}
will asymptote at either a fixed point or
a limit cycle of 2. 
Sufficient conditions for this result are: initial $\bx\in [-1,+1]^n$, $\bW=\bW^\T$, $w_{ii} \ge 0$, and $f(.)$ piecewise continuous and strictly increasing with $\lim_{\eta\to\pm\infty} f(\eta)=\pm1$. The proof is cast in terms of an 
energy function,
\begin{equation}
E(\bx) = - \frac{1}{2} \bx \bW \bx^{\T} - \bx \bb^{\T} 
+ \sum_i \int_{0}^{x_{i}} f^{-1} (\xi) d\xi .
\label{eq:energy}
\end{equation}
With $f \equiv \mathrm{tanh}$, we have the barrier function:
\begin{equation}
\rho(x_i) \equiv \int_{0}^{x_{i}} f^{-1} (\xi) d\xi  = (1+x_i) \ln (1+x_i) + (1-x_i) \ln (1-x_i)
\label{eq:barrier}
\end{equation}
To ensure a fixed point (no limit cycle > 1), asynchronous updates are sufficient because 
the solution of  $\partial E / \partial x_i = 0$ is the standard update for unit $i$ 
(Equation~\ref{eq:xiupdate}). Because the energy function
additively factorizes for units that have no direct connections, parallel updates of these units still 
ensure non-increasing energy, and hence attainment of a fixed point.

We adopt the bipartite architecture of a stacked restricted Boltzmann machine \citep{Hinton2006}, with 
bidirectional symmetric connections between adjacent layers of units and no connectivity within a 
layer (Figure~\ref{fig:1}c). We distinguish between \emph{visible} layers, which contain inputs and/or outputs of 
the net, and \emph{hidden} layers. The bipartite architecture allows for units within a layer to be updated in 
parallel while guaranteeing strictly non-increasing energy and attainment of a local energy minimum.
We thus perform layerwise updating of units, defining one \emph{iteration} as a sweep from one end of the architecture 
to the other and back. The 8-step update sequence for the architecture in Figure~\ref{fig:1}c is shown above the network.

\subsection{Convolutional Weight Constraints}

Weight constraints required for convergence can be achieved within a convolutional architecture as well (Figure~\ref{fig:1}d). 
In a feedforward convolutional architecture, the connectivity from layer $l$ to $l+1$ is represented by weights 
$\smash{\bW^{l} = \{ w_{qrab}^l \}}$, where $q$ and $r$ are channel indices in the destination ($l+1$) and source ($l$) layers, 
respectively,  and $a$ and $b$ specify the relative coordinate within the kernel, such that the weight $w_{qrab}^l$ modulates the 
input to the unit in layer $l+1$, channel $q$, absolute position $\smash{(\alpha,\beta)}$---denoted $x^{l+1}_{q\alpha\beta}$---from 
the unit $x^l_{r,\alpha+a,\beta+b}$.
If $\,\smash{\xbar{\bW}{l+1}{}=\{ \xbar{w}{l+1}{qrab} \}}$ denotes the reverse weights to channel $q$ in layer $l$ from channel $r$ in 
layer $l+1$, symmetry requires that
\begin{equation}
w^l_{q,r,a,b} = \xbar{w}{l+1}{r,q,-a,-b} ~.
\label{eq:wtconstr}
\end{equation}
This follows from the fact that the weights are translation invariant: the reverse mapping from 
${x^{l+1}_{q,\alpha,\beta}}$ to ${x^l_{r,\alpha+a,\beta+b}}$ has the same weight as from 
${x^{l+1}_{q,\alpha-a,\beta-b}}$ to ${x^l_{r,\alpha,\beta}}$, embodied in Equation \ref{eq:wtconstr}. 
Implementation of the weight constraint is simple: $\smash{\bW^{l}}$ is unconstrained, and $\smash{\xbar{\bW}{l+1}{}}$ is obtained by transposing the first two tensor dimensions of $\smash{\bW^l}$ and flipping the indices of the last two. The convolutional bipartite architecture has energy function:
% This version is correct but verbose
%\begin{align*}
% \textstyle E(\bx) = -\frac{1}{2} \sum_{l=2}^{L} \sum_{q} \bx_q^{l} \bullet \left( \bW^{l-1}_{q} * \bx^{l-1} \right)
%-\frac{1}{2} \sum_{l=1}^{L-1} &\textstyle \sum_{r} \bx_r^l \bullet \left( \xbar{\bW}{l+1}{r} * \bx^{l+1} \right)  \\
%&\textstyle + \sum_{l=1}^{L} \sum_{q,\alpha,\beta} ~\rho(x^l_{q\alpha\beta}) - b_q^l ~ x^l_{q\alpha\beta} 
%\end{align*}
\begin{equation}
%% NOTE: if we need more space on page we can insert
%\textstyle
E(\bx) = -\sum_{l=1}^{L-1} \sum_{q} \bx_q^{l+1} \bullet \left( \bW^{l}_{q} * \bx^{l} \right)
+ \sum_{l=1}^{L} \sum_{q,\alpha,\beta} ~\rho(x^l_{q\alpha\beta}) - b_q^l ~ x^l_{q\alpha\beta} 
\label{eq:enery}
\end{equation}
where $\bx^l$ is the activation in layer $l$, $\bb^l$ are the channel biases, and $\rho(.)$ is the barrier function (Equation~\ref{eq:barrier}), `$*$' is the convolution operator, and `$\bullet$' is the element-wise sum of the Hadamard product of tensors.  The factor of $\frac{1}{2}$ ordinarily found in energy functions is not present in the first term because, in contrast to Equation~\ref{eq:energy}, each second-order term in
$\bx$ appears only once. For a similar formulation in stacked restricted Boltzmann machines, see \citet{Lee2009}.


\subsection{Loss Functions}

Evidence provided to the CBAN consists of activation constraints on a subset of the visible units.
The CBAN is trained to fill-in or complete the activation pattern over 
the visible state.  The manner in which evidence constrains activations depends on the nature
of the evidence. In a scenario where all features are present but potentially noisy, one should
treat them as soft constraints that can be overridden by the model; in a scenario where
the evidence features are reliable but other features are entirely missing, one should treat
the evidence as hard constraints. 

We have focused on this latter scenario in our simulations,
although we discuss the use of soft constraints in Appendix~\ref{appendix:evidence}.
For a hard constraint, we \emph{clamp} the visible units to the value of the evidence, meaning 
that activation is set to the observed value and not allowed to change.  Energy is minimized 
conditioned on the clamped values.  One extension to clamping is to replicate all visible 
units and designate one set as input, clamped to the evidence, and one set as output, which serves as the network read out. 
We considered  using the evidence to initialize the visible state, but initialization is inadequate
to anchor the visible state and it wanders. We also considered using the evidence as a fixed bias  
on the input to the visible state, but redundancy of the bias and top-down signals from the hidden 
layer can prevent the CBAN from achieving the desired activations. 

An obvious loss function is squared error, $\mathcal{L}_{SE} = \sum_{i} ||v_i - y_i ||^2$, where
$i$ is an index over visible units, $\bv$ is the visible state, and $\by$ is the target visible state. However, this loss misses out on a key source of error. The clamped units have zero error under this loss.  Consequently, we replace $v_i$ with $\tilde{v}_i$, the value that unit $i$ would take were it unclamped, i.e., free to take on a value consistent with the hidden units driving it:
\[
\textstyle 
\mathcal{L}_{SE} = \sum_i || \tilde{v}_i - y_i || ^2 . 
\]
An alternative loss, related to the contrastive loss of the Boltzmann machine (see Appendix~\ref{appendix:loss}), explicitly aims to ensure that the energy of the current state is higher than that of the target state. With $\bx = (\by, \bh)$ being the complete state with all visible units clamped at their target values and the hidden units in some configuration $\bh$, and $\tilde{\bx} = (\tilde{\bv}, \bh)$ being the complete state with the visible units unclamped, one can define the loss
\[
\textstyle 
\mathcal{L}_{\Delta E} = E(\bx) - E(\tilde{\bx}) = 
\sum_{i} f^{-1}(\tilde{v}_i)(\tilde{v}_i - y_i) + \rho(y_i) - \rho(\tilde{v}_i) .
\]
We apply this loss by allowing the net to iterate for some number of steps given a partially clamped input, yielding a hidden state that is a plausible candidate to generate the target visible state. Note that $\rho(y_i)$ is constant and although it does not factor into the gradient
computation, it helps interpret $\mathcal{L}_{\Delta E}$: when $\mathcal{L}_{\Delta E}=0$, $\tilde{\bv}=\by$. This loss is curious in that
it is a function not just of the visible state, but, through the term $f^{-1}(\tilde{v}_i)$, it directly depends on the hidden state in the
adjacent layer and the weights between these layers.  A variant on $\mathcal{L}_{\Delta E}$ is based on the observation that the goal of
training is only to make the two energies equal, suggesting a soft hinge loss:
\[
% \textstyle 
\mathcal{L}_{\Delta E +} = \log \left( 1 + \exp(E(\bx) - E(\tilde{\bx})) \right).
\]
Both energy-based losses have an interpretation under the Boltzmann distribution: 
$\mathcal{L}_{\Delta E}$ is related to the conditional likelihood ratio of the clamped to 
unclamped visible state, and  $\mathcal{L}_{\Delta E +}$  is related to the conditional 
probability  of the clamped versus unclamped visible state:
\[
\textstyle 
\mathcal{L}_{\Delta E}  = -\log \frac{p(\by|\bh)}{p(\tilde{\bv} | \bh)} ~~~~~~~\text{and}~~~~~~~
\mathcal{L}_{\Delta E +} = -\log \frac{p(\by|\bh)}{p(\tilde{\bv}|\bh)+ p(\by | \bh)} ~.
\]
\vspace{-.12in}
\subsection{Preventing vanishing/exploding gradients}
\vspace{-.05in}
Although gradient descent is a more powerful method to train the CBAN than 
Hopfield's Hebb rule or the Boltzmann machine's contrastive loss,
vanishing and exploding gradients are a concern as with any recurrent net 
\citep{Hochreiter2001}, particularly in the CBAN which may take 50 steps to
fully relax. We address the gradient issue in two ways: through intermediate training signals and through a soft sigmoid activation function.

The aim of the CBAN is to produce a stable interpretation asymptotically.
The appropriate way to achieve this is to apply the loss once activation converges.
%If convergence takes dozens of iterations, the unrolled model becomes quite deep 
%and gradient signals are lost. 
However, the loss can be applied prior to convergence
as well, essentially training the net to achieve convergence as quickly as possible,
while also introducing loss gradients deep inside the unrolled net. 
Assume a \emph{stability criterion} $\theta$ that determines the iteration $t^*$
at which the net has effectively converged:
\[
\textstyle t^* = \min_t \left[ \max_i |x_i(t) - x_i(t-1)| < \theta \right] .
\]
Training can be logically separated into pre- and post-convergence phases, which we will refer to as \emph{transient} and 
\emph{stationary}.  In the stationary phase, the Almeida/Pineda algorithm
\citep{Pineda1987,Almeida1987} leverages the fact that activation is constant over iterations, permitting a computationally
efficient  gradient calculation with low memory requirements. In the transient phase, the loss can be injected at each step,
which is exactly the temporal-difference method TD(1) \citep{Sutton1988}. Casting training as 
temporal-difference learning, one might consider other values of $\lambda$ in TD($\lambda$); for example, TD(0) trains
the model to predict the visible state at the next time step, encouraging the model to reach the target state as 
quickly as feasible while not penalizing it for being unable to get to the target immediately. 


Any of the losses, $\mathcal{L}_{SE}$, $\mathcal{L}_{\Delta E}$, and
$\mathcal{L}_{\Delta E +}$, can be applied with a weighted mixture of training in the stationary and
transient phases. Although we do not report systematic experiments in this article, we
consistently find that transient training with $\lambda=1$ is as efficient and effective as weighted mixtures including stationary-phase-only
training, and that $\lambda=1$ outperforms any $\lambda<1$. In our results, we thus conduct simulations with transient-phase
training and $\lambda=1$.

We propose a second method of avoiding vanishing gradients specifically due to sigmoidal activation functions: a \emph{leaky sigmoid}, 
analogous to a leaky ReLU, which allows gradients to propagate through the net more freely. The leaky sigmoid has activation
and barrier functions
\begin{equation*}
f(z) = 
    \begin{cases}
    \alpha(z+1)-1 & z<-1 \\
    z & -1 \le z \le 1 \\
    \alpha(z-1)+1 & z>1\\
    \end{cases} ,~~
%~~~~\text{and}~~~~
\rho(x) = 
\vspace{.05in}
\begin{cases}
\frac{1}{2\alpha}\left[ x^2 + (1-\alpha)(1+2x)\right] & \text{if }  x < -1 \\
\frac{1}{2} x^2 & \text{if } -1 \le x \le 1 \\
\frac{1}{2\alpha}\left[ x^2 + (1-\alpha)(1-2x)\right] & \text{if }  x > 1 \
\end{cases} .
\vspace{.05in}
\end{equation*}
Parameter $\alpha$ specifies the slope of the piecewise linear function outside the $|x|<1$ interval. As $\alpha\to0$, loss gradients
become flat and the CBAN fails to train well. As $\alpha\to1$, activation magnitudes can blow up and the CBAN fails to reach a fixed point.
In Appendix~\ref{appendix:proof}, we show that convergence to a fixed point is guaranteed when
$\alpha||\bW||_{1,\infty}< 1$, where $||\bW||_{1,\infty} = \max_i ||\bw_i||_1$.
In practice, we have found that
restricting $\bW$ is unnecessary and $\alpha=0.2$ works well.


==> CBAN [ARXIV - (ICLR) 2020]/sections/03_simulations.tex <==
\section{Simulations}
We report on a series of simulation studies of increasing complexity. First, we explore fully connected bipartite attractor net (FBAN) on a bar imputation task and then supervised MNIST image completion and classification. Second, we apply CBAN to unsupervised image completion tasks on Omniglot and CIFAR-10 and compare CBAN to CBAN-variants and denoising-VAEs. Lastly, we revision CBAN for the task of super-resolution and report promising results against competing models, such as DRCN and LapSRN. Details of architectures, parameters, and training are in Appendix~\ref{appendix:arch}.

\begin{figure}[b!]
    \centering
    \includegraphics[width=5.5in]{figures/bar.pdf}
    \caption{Bar task: Input consists of $5\times5$ pixel arrays with the target being either two rows or two columns of pixels present.}
    \label{fig:bar_act}
\end{figure}
\begin{figure}[b!]
    \centering
    \includegraphics[width=5.5in]{figures/bar_weights.pdf}
    \caption{Bar task: Weights between visible and first hidden layers}
    \label{fig:bar_weights}
\end{figure}

\subsection{Bar Task} 
We studied a simple inference task on partial images that have exactly one correct interpretation.
Images are $5\times5$ binary pixel arrays consisting of two horizontal bars or two vertical bars.
Twenty distinct images exist, shown in the top row of Figure~\ref{fig:bar_act}. A subset of pixels
is provided as evidence; examples are shown in the bottom row of Figure~\ref{fig:bar_act}.  The 
task is to fill in the masked pixels. Evidence is generated such that only one consistent completion exists.
In some cases, a bar must be inferred without any white pixels as evidence (e.g., second column from the right).
In other cases, the local evidence is consistent with both vertical and horizontal bars (e.g.,
first column from left).

An FBAN with one layer of 50 hidden units is sufficient
for the task. 
%Although there are only twenty target states, there are a vast number of evidence states.
Evidence is generated randomly on each trial, and evaluating on 10k random states after training, the model 
is 99.995\% correct.  The middle row in Figure~\ref{fig:bar_act} shows the FBAN response after
one iteration.
%(one pass of activation from visible through the hidden and back to the visible). 
The net comes close 
to performing the task in a single shot, but after a second iteration of clean up and the asymptotic state is 
shown in the top row. 

Figure~\ref{fig:bar_weights} shows some visible-hidden weights learned by the FBAN.  Each 
$5\times5$ array depicts weights to/from one hidden unit. Weight sign and magnitude are indicated
by coloring and area of the square, respectively.
Units appear to select one row and one column, either with the same or opposite polarity. 
Same-polarity weights within a row or column induce coherence
among pixels. Opposite-polarity weights between a row and a column allow the pixel at the
intersection to activate either the row/column depending on the sign of the unit's activation.
%with positive weight (if the unit's
%activation is positive) or the row/column with negative weight (if the unit's
%activation is negative).


\begin{figure}[t!]
    \centering
    \includegraphics[width=5.5in]{figures/MNIST_act_main.pdf}
    \caption{MNIST completions. Row 1: target test examples, with class label coded in the bottom row.
    Row 2: completions produced by the FBAN. Row 3: Evidence with masked regions
    (including class labels) in red.
    Row 4: the top-down `dream' state produced 
    by the hidden representation.}
    \label{fig:mnist_act}
\end{figure}


\subsection{Supervised MNIST} 
We trained an FBAN with two hidden layers on a supervised version of MNIST in which the visible state consists
of a $28\times28$ array for an MNIST digit and an additional vector to code the class label. For the sake of 
graphical convenience, we allocate 28 units to the label, using the first 20 by redundantly coding the class label 
in pairs of units, and ignoring the final 8 units.  Our architecture had 812 inputs, 200 units in the first hidden layer,
and 50 units in the second. During training, all bits of the label were masked as well as one-third of image pixels.
The image was masked with thresholded Perlin coherent noise \citep{Perlin1985}, which produces missing patches that
are far more difficult to fill in than the isolated pixels produced by Bernoulli masking.

Figure~\ref{fig:mnist_act} shows evidence provided to FBAN for 20 random test set items in the third row. The red masks 
indicate unobserved pixels; the other pixels are clamped in the visible state. The unobserved pixels include those 
representing the class label, coded in the bottom row of the pixel array. The top row of the Figure shows the target
visible representation, with class labels indicated by the isolated white pixels.
Even though the training loss treats all pixels as equivalent, the FBAN does learn to
classify unlabeled images. On the test set, the model achieves a classification
accuracy of 87.5\% on Perlin-masked test images and 89.9\% on noise-free test images. Note
that the 20 pixels indicating class membership are no different than any other missing pixels in the input.
The model learns to classify by virtue of the systematic relationship between images and labels. We can train the
model with fully observed images and fully unobserved labels, and its performance is like that of any fully-connected
MNIST classifier, achieving an accuracy of 98.5\%.

The FBAN does an excellent job of filling in missing features in Figure~\ref{fig:mnist_act}
and in further examples in Appendix~\ref{appendix:results}.
The FBAN's interpretations of the input seem to be respectable in comparison to other
recent recurrent associative memory models (Figures~\ref{fig:mnist_weights}a,b).
We mean no disrespect of other research efforts---which have very different foci than ours---but merely wish to indicate
we are obtaining state-of-the-art results for associative memory models. Figure~\ref{fig:mnist_weights}c shows some 
weights between visible and hidden units. Note that the weights link image pixels with multiple digit labels.
These weights stand apart from the usual hidden representations found in feedforward classification networks.



%%% FIGURE
%%% ============================
\begin{figure}[htp]
  \centering
    \includegraphics[width=5.5in]{figures/omniglot_quant_combo_v2.pdf}
    \caption{Omniglot image completion comparison examples (left) and quantitative results (right). The top two rows of the examples show the target image and the evidence provided to the model (with missing pixels depicted in red), respectively. The subsequent rows show the image completions produced by CBAN, CBAN-asym, CBAN-noTD, and the denoising VAE. The quantitative measures evaluate each model on PSNR and SSIM metrics; black lines indicate $+1$ standard error of the mean.}
    \label{fig:omniglot_comparison}
\end{figure}
%%% ============================


\subsection{Unsupervised Omniglot} 
We trained a CBAN with the Omniglot images \citep{omniglot}.
Omniglot consists of multiple instances of 1623 characters from 50 different
alphabets. The CBAN has one visible layer containing the character image, $28\times28\times1$, and three
successive hidden layers with dimensions $28\times28\times128$, $14\times14\times256$, and $7\times7\times256$, 
all with average pooling between the layers and filters of  size $3\times3$.
Other network parameters and training details are presented in Appendix~\ref{appendix:arch}.
To experiment with a different type of masking, we used random square patches of diameter 3--6, which remove on average roughly 30\% of the white pixels in the image.

%Reconstructions of masked characters from the test set (Figure~\ref{fig:omniglot_comparison}, left). 


We compared our CBAN to variants with critical properties removed: one without 
weight symmetry  (\emph{CBAN-asym}) and one in which the TD(1) training procedure 
is substituted for a standard squared loss at the final step (\emph{CBAN-noTD}). 
We also compare to a convolutional denoising VAE (\emph{CD-VAE}), which takes the
masked image as input and outputs the completion.
The CBAN with symmetric weights reaches a fixed point,
%in a mean of 43 iterations, 
whereas CBAN-asym appears to attain limit cycles of 2-10 iterations.
Qualitatively, CBAN produces the best image reconstructions 
(Figure~\ref{fig:omniglot_comparison}). CBAN-asym and CBAN-noTD tend to hallucinate
additional strokes; and CBAN-noTD and CD-VAE produce less crisp edges.
Quantitatively, we assess models with two measures of reconstruction quality,
peak signal-to-noise ratio (\emph{PSNR})  and structural similarity 
\citep[\emph{SSIM}, ][]{ssim}; larger is better on each measure. 
CBAN is strictly superior to the alternatives on both measures (Figure~\ref{fig:omniglot_comparison}, right panel).
%CBAN completions combine the clamped evidence pixels with the patterns filled in by the model (the `dream' state). 
CBAN completions are not merely memorized instances; the CBAN has learned structural regularities of the images, allowing it to fill in big gaps in images that---with the missing pixels---are typically uninterpretable by both classifiers and humans. 
Additional CBAN image completion examples for Omniglot can be found in Appendix~\ref{appendix:results}.

%%% FIGURE
%%% ============================
\begin{figure}[b!]
  \centering
    \includegraphics[width=5.5in]{figures/cifar_quant_combo.pdf}
    \caption{CIFAR-10 image completion comparison examples (left) and quantitative results (right). Layout identical to that of Figure \ref{fig:omniglot_comparison}.}
    \label{fig:cifar_qual_quant}
\end{figure}
%%% ============================




\subsection{Unsupervised CIFAR-10} 
We trained a CBAN with one visible and three hidden layers on CIFAR-10 images.
The visible layer is the size of the input image, $32\times32\times3$. The 
successive hidden  layers had dimensions $32\times32\times40$, $16\times16\times120$, 
and $8\times8\times440$, all with filters of size $3\times3$
and average pooling between the hidden layers.
Further details of architecture and training can be found in Appendix~\ref{appendix:arch}. 
Figure~\ref{fig:cifar_qual_quant} shows qualitative and quantitative comparisons
of alternative models. Here, CBAN-asym performs about the same as CBAN.
However, CBAN-asym typically attains bi-phasic limit cycles, and CBAN-asym
sometimes produces splotchy artifacts in background regions (e.g., third image 
from left). CBAN-noTD and the CD-VAE are clearly inferior to CBAN. 
Additional CBAN image completions can be found in Appendix~\ref{appendix:results}.

\subsection{Super-resolution} 
Deep learning models have proliferated in many domains of image processing, perhaps none more than image super-resolution,
which is concerned with recovering a high-resolution image from a low-resolution image. Many specialized architectures
have been developed, and although common test data sets exist, comparisons are not as simple as one would hope due 
to subtle differences in methodology. (For example, even the baseline method, bicubic interpolation, yields different results 
depending on the implementation.) We set out to explore the feasibility of using CBANs for super-resolution.
Our architecture processes $40\times40$ color image
patches, and the visible state included both the low- and high-resolution images, with the low-resolution version clamped
and the high-resolution version read out from the net.
Details can be found in Appendix~\ref{appendix:arch}.

%% Bicubic interpolation algorithm difference (Matlab vs. Cv2) note:
%% OpenCV and Matlab have different bicubic interpolation algorithms, yielding different results -- claims have been made that Matlab's version is more accurate for things like SSIM, but OpenCV is better for PSNR? Either way, we used the OpenCV implementation, whereas the papers we are comparing to used the Matlab implementation; consequently, the baselines for bicubic are different, with our SSIM values being a smidgen lower.


Table~\ref{table:sr} presents two measures of performance, SSIM and PSNR, for the CBAN and various published alternatives. CBAN beats the baseline, bicubic interpolation, on both
measures, and performs well on SSIM against some leading contenders (even
beating LapSRN and DRCN on \textit{Set14} and \textit{Urban100}), but poorly
on PSNR. It is common for PSNR and SSIM to be in opposition: SSIM rewards crisp edges, 
PSNR rewards averaging toward the mean.  The border sharpening and contrast enhancement 
that produce good perceptual quality and a high SSIM score (see Figure~\ref{fig:sr}) 
are due to the fact that CBAN comes to an interpretation of the images: it
imposes edges and textures in order to make the features mutually consistent.
We believe that CBAN warrants further investigation for super-resolution; regardless
of whether it becomes the winner in this competitive field, one can argue that it is
performing a different type of computation than feedforward models like LapSRN and DRCN.


\begin{table}[t]
    \small \centering
\begin{tabular}{llllll} \toprule 
 & Algorithm      & \begin{tabular}[c]{@{}l@{}}Set5\\ PSNR / SSIM\end{tabular} & \begin{tabular}[c]{@{}l@{}}Set14\\ PSNR / SSIM\end{tabular} & \begin{tabular}[c]{@{}l@{}}BSD100\\ PSNR / SSIM\end{tabular} & \begin{tabular}[c]{@{}l@{}}Urban100\\ PSNR / SSIM\end{tabular} \\ \midrule
 & Bicubic (baseline) & 32.21 / 0.921 & 29.21 / 0.911 & 28.67 / 0.810 & 25.63 / 0.827 \\
 & DRCN \citep{KimLeeLee2016} & 37.63 / 0.959& 32.94 / 0.913& 31.85 / 0.894& 30.76 / 0.913\\
 & LapSRN \citep{Lai2018}   & 37.52 / 0.959 & 33.08 / 0.913 & 31.80 / 0.895 & 30.41 / 0.910 \\
 & CBAN (ours) & 34.18 / 0.947 & 30.79 / \color{red}0.953\color{black}  & 30.12 / 0.872 &  27.49 / \color{red}0.915\color{black} \\ %\bottomrule
\end{tabular}
\caption{Quantitative benchmark presenting average PSNR/SSIMs for scale factor $\times$2 on four test sets. \color{red}Red \color{black} indicates superior performance of CBAN. CBAN consistently outperforms baseline Bicubic.}
\label{table:sr}
\end{table}

\begin{figure}[t]
\vspace{-.04in}
    \centering
    %\includegraphics[width=5.5in]{figures/SR_figure_3_green.pdf}
    %\includegraphics[width=5.5in]{figures/test.png}
    % new option
    %\includegraphics[width=5.5in]{figures/SR_figure_4.png}
    \includegraphics[width=5.5in]{figures/SR_figure_Mozer.pdf}
    \caption{Examples of super-resolution, with the columns in a given image group 
    comparing high-resolution ground truth, CBAN, and bicubic interpolation (baseline
    method).}
    \label{fig:sr}
    \vspace{-.06in}
\end{figure}



==> CBAN [ARXIV - (ICLR) 2020]/sections/04_discussion.tex <==

\vspace{-.1in}
\section{Discussion}
\vspace{-.06in}

% Our investigations support the value of CBANs as part of the modern deep learning toolbox.
% ^^ too strong of a claim that the N*IPS reviewers didn't seem to like very much?
In comparison to recent published results on image completion with attractor networks, 
our CBAN produces far more impressive results (see Appendix, Figure 8, for a contrast).
%Although recurrent nets are not typically used for (attention-free) vision,
The computational cost and challenge of training CBANs is no greater than those 
of training deep feedforward nets.
CBANs seem to produce crisp images, on par with those produced by generative (e.g., energy- and flow-based) models.
CBANs have potential to be applied in many contexts involving data interpretation,
with the virtue that  the computational resources they bring to bear on a task is 
dynamic and dependent on the difficulty of interpreting a given input.
%Although CBANs lack the probabilistic semantics of some generative models, their power
%is their generality and potential to be applied in many contexts involving data interpretation.
Although this article has focused on convolutional networks that have attractor dynamics \emph{between} levels of
representation, we have recently recognized the value of architectures that are fundamentally feedforward with
attractor dynamics \emph{within} a level. Our current research explores this variant of the CBAN as a biologically plausible account of intralaminar lateral inhibition.

%Our convolutional layer is a lattice of dimensions
%$n_f \times n_x \times n_y$, where 
%$n_f$ is the number of filters,
%$n_x$ is the horizontal spatial extent,  and
%$n_y$ is the vertical spatial extent.
%We will build a recurrent network which, when unfolded in time, will map from
%this layer to a layer with the
%same dimensionality via a convolutional operator with patch size
%$n_f \times (2n_r+1) \times (2n_r+1)$, where $n_r$ is the radius of the patch.
%The recurrent mapping will be determined by a set of weights, 
%$W = \{ w_{efab} \}$, where $w_{efab}$ refers to the connection feeding into
%unit $(x,y,f)$ from unit $(x+a,y+b,e)$, for every $x$ and $y$ on the lattice.
%$W$ has dimensionality $n_f \times n_f \times (2n_r+1) \times (2n_r+1)$.
%To simplify notation without any loss of generality, we will assume $x=y=0$.
%
%If $w_{efab}$ specifies the connection $(a,b,e) \to (0,0,f)$, then we require 
%this weight to be symmetric with the connection $(0,0,f)\to(a,b,e)$,
%or by normalizing with a constant offset, $(-a,-b,f)\to (0,0,e)$, i.e., 
%\[
%w_{e,f,a,b} = w_{f,e,-a,-b}.
%\]
%Our challenge is how to efficiently enforce this constraint, or how
%to express the underlying parameters and how they map to $W$. 

%Remember, we also need to enforce the self-connection constraint $w_{f,f,0,0}\ge0$ for all $f$.



%\begin{table}
%  \caption{Sample table title}
%  \label{sample-table}
%  \centering
%  \begin{tabular}{lll}
%    \toprule
%    \multicolumn{2}{c}{Part}           %        \\
%    \cmidrule(r){1-2}
%    Name     & Description     & Size %($\mu$m) \\
%    \midrule
%    Dendrite & Input terminal  & %$\sim$100     \\
%    Axon     & Output terminal & %$\sim$10      \\
%    Soma     & Cell body       & up to %$10^6$  \\
%    \bottomrule
%  \end{tabular}
%\end{table}

% REMOVED FOR SUBMISSION
%\subsubsection{Acknowledgements}
%We gratefully acknowledge the contributions of Aditya Thygarangan who conducted initial experiments with attractor networks that convinced us to 
%pursue this line of research. Thanks also to Been Kim for guidance on the use of Perlin Noise, and to David Grangier, 
%Tyler Scott and Karl Ridgeway for helpful feedback on the research.


%\bibliographystyle{apa}
\bibliographystyle{abbrvnat}
\bibliography{CBANet}

\input{appendix/appendix.tex}


==> CBAN [ARXIV - (ICLR) 2020]/sections/packages.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[hyphens]{url}            % simple URL typesetting
\usepackage[colorlinks=true,citecolor=blue]{hyperref}       % hyperlinks
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{enumitem}
\usepackage{bm}
\usepackage{float}
\usepackage{caption}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{bbold}
\usepackage{relsize}
\usepackage{multicol}
\usepackage{adjustbox}
\usepackage{wrapfig}

==> sections/packages.tex <==
\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage[hyphens]{url}            % simple URL typesetting
\usepackage[colorlinks=true,citecolor=blue]{hyperref}       % hyperlinks
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsmath,amsfonts,amssymb}
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{enumitem}
\usepackage{bm}
\usepackage{float}
\usepackage{caption}
\usepackage{xcolor}
\usepackage{graphicx}
\usepackage{bbold}
\usepackage{relsize}
\usepackage{multicol}
\usepackage{adjustbox}
\usepackage{wrapfig}
